Wolf 503 b: Characterization of a Sub-Neptune Orbiting a Metal-Poor K Dwarf

Using radial velocity measurements from four instruments, we report the mass and density of a $2.043\pm0.069 ~\rm{R}_{\oplus}$ sub-Neptune orbiting the quiet K-dwarf Wolf 503 (HIP 67285). In addition, we present improved orbital and transit parameters by analyzing previously unused short-cadence $K2$ campaign 17 photometry and conduct a joint radial velocity-transit fit to constrain the eccentricity at $0.41\pm0.05$. The addition of a transit observation by $Spitzer$ also allows us to refine the orbital ephemeris in anticipation of further follow-up. Our mass determination, $6.26^{+0.69}_{-0.70}~\rm{M}_{\odot}$, in combination with the updated radius measurements, gives Wolf 503 b a bulk density of $\rho = 2.92\pm ^{+0.50}_{-0.44}$ $\rm{g}~\rm{cm}^{-3}$. Using interior composition models, we find this density is consistent with an Earth-like core with either a substantial $\rm{H}_2\rm{O}$ mass fraction ($45^{+19.12}_{-16.15}\%$) or a modest H/He envelope ($0.5\pm0.28\%$). The low H/He mass fraction, along with the old age of Wolf 503 ($11\pm2$ Gyrs), makes this sub-Neptune an opportune subject for testing theories of XUV-driven mass loss while the brightness of its host ($J=8.3$ mag) makes it an attractive target for transmission spectroscopy.

==> authors.tex <==
\correspondingauthor{Alex S.\ Polanski}
\email{aspolanski@ku.edu}

\author{Alex S. Polanski} 
\affil{Department of Physics and Astronomy, University of Kansas, Lawrence, KS 66045, USA}

\author{Ian J.~M.\ Crossfield}
\affil{Department of Physics and Astronomy, University of Kansas, Lawrence, KS 66045, USA}
\nocollaboration{2}
%%%%%%%%%%%%%%%%%%%%%% Collaboration Leads and Major Contributors %%%%%%%%%%%%%%%%%%%%%%%

\author[0000-0002-0040-6815]{Jennifer~A.~Burt}
\affiliation{Jet Propulsion Laboratory, California Institute of Technology, 4800 Oak Grove Drive, Pasadena, CA 91109, USA}

\author{Grzegorz Nowak}
\affiliation{Instituto de Astrofísica de Canarias, Vía Láctea s/n, 38205 La
Laguna, Tenerife, Spain}
\affiliation{Departamento de Astrofísica, Universidad de La Laguna, Spain}

\author{Mercedes Lopez-Morales}
\affiliation{Center for Astrophysics | Harvard & Smithsonian, 60 Garden Street, Cambridge, MA, 02138, USA}

\author[0000-0001-7254-4363]{Annelies Mortier}
\affiliation{Astrophysics Group, Cavendish Laboratory, University of Cambridge, J.J. Thomson Avenue, Cambridge CB3 0HE, UK}
\affiliation{Kavli Institute for Cosmology, University of Cambridge, Madingley Road, Cambridge CB3 0HA, UK}

\author{Ennio Poretti}
\affiliation{Fundaci\'{o}n Galileo Galilei -- INAF, Rambla Jos\'{e} Ana Fernandez P\'{e}rez 7, 38712 -- Bre\~{n}a Baja, Spain}

\nocollaboration{5}
%%%%%%%%%%%%%%%%%%%%%% Contributors (Alphabetical Order) %%%%%%%%%%%%%%%%%%%%%%%

\author[0000-0003-0012-9093]{Aida Behmard}
\affiliation{Division of Geological and Planetary Sciences, California Institute of Technology, Pasadena, CA 91125, USA}

\author{Bj\"orn Benneke}
\affiliation{Departement de Physique, and Institute for Research on Exoplanets, Universite de Montreal, Montreal, H3T J4, Canada}

\author{Sarah Blunt}
\affiliation{Department of Astronomy, California Institute of Technology, Pasadena, CA 91125, USA}

\author[0000-0003-1305-3761]{R.~Paul~Butler}
\affiliation{Earth \& Planets Laboratory, Carnegie Institution for Science, 5241 Broad Branch Road, NW, Washington, DC 20015, USA}

\author[0000-0003-1125-2564]{Ashley Chontos}
\altaffiliation{NSF Graduate Research Fellow}
\affiliation{Institute for Astronomy, University of Hawai'i, 2680 Woodlawn Drive, Honolulu, HI 96822, USA}

\author{Rosario Cosentino}
\affiliation{Fundaci\'{o}n Galileo Galilei -- INAF, Rambla Jos\'{e} Ana Fernandez P\'{e}rez 7, 38712 -- Bre\~{n}a Baja, Spain}
\affiliation{INAF - Osservatorio Astrofisico di Catania, Catania, Italy}

\author[0000-0002-5226-787X]{Jeffrey~D.~Crane}
\affiliation{The Observatories of the Carnegie Institution for Science, 813 Santa Barbara Street, Pasadena, CA 91101, USA}

\author{Xavier Dumusque}
\affiliation{Observatoire de Gen\`eve, 51 Chemin de Pegasi, 1290 Versoix, Switzerland}

\author{Benjamin J.\ Fulton}
\affil{Caltech/IPAC-NASA Exoplanet Science Institute, 770 S. Wilson Ave, Pasadena, CA 91106, USA}

\author{Adriano Ghedina}
\affiliation{Fundaci\'{o}n Galileo Galilei -- INAF, Rambla Jos\'{e} Ana Fernandez P\'{e}rez 7, 38712 -- Bre\~{n}a Baja, Spain}

\author{Varoujan Gorjian}
\affiliation{Jet Propulsion Laboratory, California Institute of Technology, 4800 Oak Grove Drive, Pasadena, CA 91109, USA}

\author[0000-0003-4976-9980]{Samuel K. Grunblatt}
\altaffiliation{Kalbfleisch Fellow}
\affiliation{American Museum of Natural History, 200 Central Park West, Manhattan, NY 10024, USA}
\affiliation{Center for Computational Astrophysics, Flatiron Institute, 162 5$^\text{th}$ Avenue, Manhattan, NY 10010, USA}

\author{Avet Harutyunyan}
\affiliation{Fundaci\'{o}n Galileo Galilei -- INAF, Rambla Jos\'{e} Ana Fernandez P\'{e}rez 7, 38712 -- Bre\~{n}a Baja, Spain}

\author[0000-0001-8638-0320]{Andrew W.\ Howard}
\affil{Department of Astronomy, California Institute of Technology, Pasadena, CA 91125, USA}

\author{Chelsea X.Huang}
\affil{Department of Physics, and Kavli Institute for Astrophysics and Space Research, Massachusetts Institute of Technology, Cambridge, MA 02139, USA}

\author{Howard Isaacson}
\affil{Department of Astronomy, University of California, Berkeley, CA 94720}

\author{Molly R.\ Kosiarek}
\altaffiliation{NSF Graduate Research Fellow}
\affil{Department of Astronomy and Astrophysics, University of California, Santa Cruz, CA 95064, USA}

\author{David W.\ Latham}
\affil{Center for Astrophysics, 60 Garden Street, Cambridge, MA 02138, USA}

\author{Rafael Luque}
\affiliation{Instituto de Astrofísica de Canarias, Vía Láctea s/n, 38205 La Laguna, Tenerife, Spain}
\affiliation{Departamento de Astrofísica, Universidad de La Laguna, Spain}

\author{Aldo F. Martinez Fiorenzano}
\affiliation{Fundaci\'{o}n Galileo Galilei -- INAF, Rambla Jos\'{e} Ana Fernandez P\'{e}rez 7, 38712 -- Bre\~{n}a Baja, Spain}

\author{Michel Mayor}
\affiliation{Observatoire de Gen\`eve, 51 Chemin de Pegasi, 1290 Versoix, Switzerland}

\author[0000-0002-4535-6241]{Sean M. Mills}
\affiliation{Department of Astronomy, California Institute of Technology, Pasadena, CA 91125, USA}

\author{Emilio Molinari}
\affiliation{INAF - Osservatorio Astronomico di Cagliari, Selargius, Italy}

\author[0000-0002-4019-3631]{Evangelos Nagel}
\affiliation{Thüringer Landessternwarte Tautenburg, Sternwarte 5, 07778 Tautenburg, Germany}
\affiliation{Hamburger Sternwarte, Gojenbergsweg 112, 21029 Hamburg, Germany}

\author[0000-0003-0987-1593]{Enric Pall\'{e}}
\affiliation{Instituto de Astrofísica de Canarias, Vía Láctea s/n, 38205 La
Laguna, Tenerife, Spain}
\affiliation{Departamento de Astrofísica, Universidad de La Laguna, Spain}

\author[0000-0003-0967-2893]{Erik A.\ Petigura}
\affil{Department of Physics and Astronomy, University of California, Los Angeles, CA 90095, USA}

\author{Stephen~A.~Shectman}
\affiliation{The Observatories of the Carnegie Institution for Science, 813 Santa Barbara Street, Pasadena, CA 91101, USA}

\author[0000-0002-7504-365X]{Alessandro Sozzetti}
\affiliation{INAF - Osservatorio Astrofisico di Torino, Strada Osservatorio 20, I-10025 Pino Torinese (TO), Italy}

\author{Johanna~K.~Teske}
\affiliation{Earth \& Planets Laboratory, Carnegie Institution for Science, 5241 Broad Branch Road, NW, Washington, DC 20015, USA}

\author[0000-0002-6937-9034]{Sharon Xuesong Wang}
\affiliation{Department of Astronomy, Tsinghua University, Beijing 100084, People's Republic of China}

\author[0000-0002-3725-3058]{Lauren M. Weiss}
\affiliation{Institute for Astronomy, University of Hawai'i, 2680 Woodlawn Drive, Honolulu, HI 96822, USA}

\nocollaboration{31}
